Wave dispersion in pulsar plasma: 2. Pulsar frame

Wave dispersion in a pulsar plasma is discussed emphasizing the relevance of different inertial frames, notably the plasma rest frame ${\cal K}$ and the pulsar frame ${\cal K}'$ in which the plasma is streaming with speed $\beta_{\rm s}$. The effect of a Lorentz transformation on both subluminal, $|z|<1$, and superluminal, $|z|>1$, waves is discussed. It is argued that the preferred choice for a relativistically streaming distribution should be a Lorentz-transformed J\"uttner distribution; such a distribution is compared with other choices including a relativistically streaming Gaussian distribution. A Lorentz transformation of the dielectric tensor is written down, and used to derive an explicit relation between the relativistic plasma dispersion functions in ${\cal K}$ and ${\cal K}'$. It is shown that the dispersion equation can be written in an invariant form, implying a one-to-one correspondence between wave modes in any two inertial frames. Although there are only three modes in the plasma rest frame, it is possible for backward-propagating or negative-frequency solutions in ${\cal K}$ to transform into additional forward-propagating, positive-frequency solutions in ${\cal K}'$ that may be regarded as additional modes.

==> fig1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{018}[tc][tc]{\matlabtextA $ z $}%
\psfrag{019}[bc][bc]{\matlabtextA $ z' $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 4$}%
\psfrag{001}[ct][ct]{\matlabtextB $\matlabfragNegXTick 3$}%
\psfrag{002}[ct][ct]{\matlabtextB $\matlabfragNegXTick 2$}%
\psfrag{003}[ct][ct]{\matlabtextB $\matlabfragNegXTick 1$}%
\psfrag{004}[ct][ct]{\matlabtextB $0$}%
\psfrag{005}[ct][ct]{\matlabtextB $1$}%
\psfrag{006}[ct][ct]{\matlabtextB $2$}%
\psfrag{007}[ct][ct]{\matlabtextB $3$}%
\psfrag{008}[ct][ct]{\matlabtextB $4$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextB $-4$}%
\psfrag{010}[rc][rc]{\matlabtextB $-3$}%
\psfrag{011}[rc][rc]{\matlabtextB $-2$}%
\psfrag{012}[rc][rc]{\matlabtextB $-1$}%
\psfrag{013}[rc][rc]{\matlabtextB $0$}%
\psfrag{014}[rc][rc]{\matlabtextB $1$}%
\psfrag{015}[rc][rc]{\matlabtextB $2$}%
\psfrag{016}[rc][rc]{\matlabtextB $3$}%
\psfrag{017}[rc][rc]{\matlabtextB $4$}%
%
%% </ytick>

==> fig10.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11.00}{11.00}\selectfont\strut}%
\psfrag{016}[tc][tc]{\matlabtextA $ {\rm sgn}(z')\log_{10}(\gamma'_\phi) $}%
\psfrag{017}[bc][bc]{\matlabtextA $ W'(z') $}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10.00}{10.00}\selectfont\strut}%
\psfrag{015}[bc][bc]{\matlabtextB $ \times 10^3 $}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{10.00}{10.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegTickNoWidth 1$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $1$}%
\psfrag{003}[ct][ct]{\matlabtextC $2$}%
\psfrag{004}[ct][ct]{\matlabtextC $3$}%
\psfrag{005}[ct][ct]{\matlabtextC $4$}%
\psfrag{006}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $-2$}%
\psfrag{008}[rc][rc]{\matlabtextC $-1.5$}%
\psfrag{009}[rc][rc]{\matlabtextC $-1$}%
\psfrag{010}[rc][rc]{\matlabtextC $-0.5$}%
\psfrag{011}[rc][rc]{\matlabtextC $0$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{013}[rc][rc]{\matlabtextC $1$}%
\psfrag{014}[rc][rc]{\matlabtextC $1.5$}%
%
%% </ytick>

==> fig11.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{019}[tc][tc]{\matlabtextA $ {\rm sgn}(z')\log_{10}(\gamma'_\phi) $}%
\psfrag{020}[bc][bc]{\matlabtextA $ \omega'/\omega'_{\rm p0} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 2$}%
\psfrag{001}[ct][ct]{\matlabtextB $\matlabfragNegXTick 1$}%
\psfrag{002}[ct][ct]{\matlabtextB $0$}%
\psfrag{003}[ct][ct]{\matlabtextB $1$}%
\psfrag{004}[ct][ct]{\matlabtextB $2$}%
\psfrag{005}[ct][ct]{\matlabtextB $3$}%
\psfrag{006}[ct][ct]{\matlabtextB $4$}%
\psfrag{007}[ct][ct]{\matlabtextB $5$}%
\psfrag{008}[ct][ct]{\matlabtextB $6$}%
\psfrag{009}[ct][ct]{\matlabtextB $7$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextB $10^{-4}$}%
\psfrag{011}[rc][rc]{\matlabtextB $10^{-3}$}%
\psfrag{012}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{013}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{014}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{015}[rc][rc]{\matlabtextB $10^{1}$}%
\psfrag{016}[rc][rc]{\matlabtextB $10^{2}$}%
\psfrag{017}[rc][rc]{\matlabtextB $10^{3}$}%
\psfrag{018}[rc][rc]{\matlabtextB $10^{4}$}%
%
%% </ytick>

==> fig2a.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{014}[tc][tc]{\matlabtextA $ u $}%
\psfrag{015}[bc][bc]{\matlabtextA $ g_\alpha(u) $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $$}%
\psfrag{001}[ct][ct]{\matlabtextB $\matlabfragNegXTick 40$}%
\psfrag{002}[ct][ct]{\matlabtextB $$}%
\psfrag{003}[ct][ct]{\matlabtextB $\matlabfragNegXTick 20$}%
\psfrag{004}[ct][ct]{\matlabtextB $$}%
\psfrag{005}[ct][ct]{\matlabtextB $0$}%
\psfrag{006}[ct][ct]{\matlabtextB $$}%
\psfrag{007}[ct][ct]{\matlabtextB $20$}%
\psfrag{008}[ct][ct]{\matlabtextB $$}%
\psfrag{009}[ct][ct]{\matlabtextB $40$}%
\psfrag{010}[ct][ct]{\matlabtextB $$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextB $0$}%
\psfrag{012}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{013}[rc][rc]{\matlabtextB $1$}%
%
%% </ytick>

==> fig2b.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{010}[tc][tc]{\matlabtextA $ u $}%
\psfrag{011}[bc][bc]{\matlabtextA $ g_\alpha(u) $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $ 10^{-1} $}%
\psfrag{001}[ct][ct]{\matlabtextB $ 10^{0} $}%
\psfrag{002}[ct][ct]{\matlabtextB $ 10^{1} $}%
\psfrag{003}[ct][ct]{\matlabtextB $ 10^{2} $}%
\psfrag{004}[ct][ct]{\matlabtextB $ 10^{3} $}%
\psfrag{005}[ct][ct]{\matlabtextB $ 10^{4} $}%
\psfrag{006}[ct][ct]{\matlabtextB $ 10^{5} $}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextB $0$}%
\psfrag{008}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{009}[rc][rc]{\matlabtextB $1$}%
%
%% </ytick>

==> fig3a.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{010}[tc][tc]{\matlabtextA $ u $}%
\psfrag{011}[bc][bc]{\matlabtextA $ g_\alpha(u) $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 60$}%
\psfrag{001}[ct][ct]{\matlabtextB $\matlabfragNegXTick 40$}%
\psfrag{002}[ct][ct]{\matlabtextB $\matlabfragNegXTick 20$}%
\psfrag{003}[ct][ct]{\matlabtextB $0$}%
\psfrag{004}[ct][ct]{\matlabtextB $20$}%
\psfrag{005}[ct][ct]{\matlabtextB $40$}%
\psfrag{006}[ct][ct]{\matlabtextB $60$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextB $0$}%
\psfrag{008}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{009}[rc][rc]{\matlabtextB $1$}%
%
%% </ytick>

==> fig3b.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{009}[tc][tc]{\matlabtextA $ u $}%
\psfrag{010}[bc][bc]{\matlabtextA $ g_\alpha(u) $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $100$}%
\psfrag{002}[ct][ct]{\matlabtextB $200$}%
\psfrag{003}[ct][ct]{\matlabtextB $300$}%
\psfrag{004}[ct][ct]{\matlabtextB $400$}%
\psfrag{005}[ct][ct]{\matlabtextB $500$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $0$}%
\psfrag{007}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{008}[rc][rc]{\matlabtextB $1$}%
%
%% </ytick>

==> fig4.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{009}[tc][tc]{\matlabtextA $ u $}%
\psfrag{010}[bc][bc]{\matlabtextA $ g_\alpha(u) $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $100$}%
\psfrag{002}[ct][ct]{\matlabtextB $200$}%
\psfrag{003}[ct][ct]{\matlabtextB $300$}%
\psfrag{004}[ct][ct]{\matlabtextB $400$}%
\psfrag{005}[ct][ct]{\matlabtextB $500$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $0$}%
\psfrag{007}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{008}[rc][rc]{\matlabtextB $1$}%
%
%% </ytick>

==> fig5a.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{010}[tc][tc]{\matlabtextA $ u $}%
\psfrag{011}[bc][bc]{\matlabtextA $ g_{\rm cs}(u) $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextB $\matlabfragNegXTick 50$}%
\psfrag{002}[ct][ct]{\matlabtextB $0$}%
\psfrag{003}[ct][ct]{\matlabtextB $50$}%
\psfrag{004}[ct][ct]{\matlabtextB $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextB $0$}%
\psfrag{006}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{007}[rc][rc]{\matlabtextB $1$}%
\psfrag{008}[rc][rc]{\matlabtextB $1.5$}%
\psfrag{009}[rc][rc]{\matlabtextB $2$}%
%
%% </ytick>

==> fig5b.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{010}[tc][tc]{\matlabtextA $ u $}%
\psfrag{011}[bc][bc]{\matlabtextA $ g_{\rm cs}(u) $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 10$}%
\psfrag{001}[ct][ct]{\matlabtextB $\matlabfragNegXTick 5$}%
\psfrag{002}[ct][ct]{\matlabtextB $0$}%
\psfrag{003}[ct][ct]{\matlabtextB $5$}%
\psfrag{004}[ct][ct]{\matlabtextB $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextB $0.8$}%
\psfrag{006}[rc][rc]{\matlabtextB $0.85$}%
\psfrag{007}[rc][rc]{\matlabtextB $0.9$}%
\psfrag{008}[rc][rc]{\matlabtextB $0.95$}%
\psfrag{009}[rc][rc]{\matlabtextB $1$}%
%
%% </ytick>

==> fig6a.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{025}[tc][tc]{\matlabtextA $ u $}%
\psfrag{026}[bc][bc]{\matlabtextA $ g(u) $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $$}%
\psfrag{002}[ct][ct]{\matlabtextB $200$}%
\psfrag{003}[ct][ct]{\matlabtextB $$}%
\psfrag{004}[ct][ct]{\matlabtextB $400$}%
\psfrag{005}[ct][ct]{\matlabtextB $$}%
\psfrag{009}[ct][ct]{\matlabtextB $\matlabfragNegXTick 100$}%
\psfrag{010}[ct][ct]{\matlabtextB $$}%
\psfrag{011}[ct][ct]{\matlabtextB $0$}%
\psfrag{012}[ct][ct]{\matlabtextB $$}%
\psfrag{013}[ct][ct]{\matlabtextB $100$}%
\psfrag{014}[ct][ct]{\matlabtextB $$}%
\psfrag{015}[ct][ct]{\matlabtextB $200$}%
\psfrag{016}[ct][ct]{\matlabtextB $$}%
\psfrag{017}[ct][ct]{\matlabtextB $300$}%
\psfrag{018}[ct][ct]{\matlabtextB $$}%
\psfrag{019}[ct][ct]{\matlabtextB $400$}%
\psfrag{020}[ct][ct]{\matlabtextB $$}%
\psfrag{021}[ct][ct]{\matlabtextB $500$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $0.08$}%
\psfrag{007}[rc][rc]{\matlabtextB $0.1$}%
\psfrag{008}[rc][rc]{\matlabtextB $0.12$}%
\psfrag{022}[rc][rc]{\matlabtextB $0$}%
\psfrag{023}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{024}[rc][rc]{\matlabtextB $1$}%
%
%% </ytick>

==> fig6b.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[tl][tl]{\matlabtextA $ \times 10^{-3} $}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{021}[tc][tc]{\matlabtextB $ u $}%
\psfrag{022}[bc][bc]{\matlabtextB $ g(u) $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $$}%
\psfrag{002}[ct][ct]{\matlabtextC $200$}%
\psfrag{003}[ct][ct]{\matlabtextC $$}%
\psfrag{004}[ct][ct]{\matlabtextC $400$}%
\psfrag{005}[ct][ct]{\matlabtextC $$}%
\psfrag{010}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{011}[ct][ct]{\matlabtextC $0$}%
\psfrag{012}[ct][ct]{\matlabtextC $100$}%
\psfrag{013}[ct][ct]{\matlabtextC $200$}%
\psfrag{014}[ct][ct]{\matlabtextC $300$}%
\psfrag{015}[ct][ct]{\matlabtextC $400$}%
\psfrag{016}[ct][ct]{\matlabtextC $500$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $9.6$}%
\psfrag{007}[rc][rc]{\matlabtextC $9.8$}%
\psfrag{008}[rc][rc]{\matlabtextC $10$}%
\psfrag{009}[rc][rc]{\matlabtextC $10.2$}%
\psfrag{017}[rc][rc]{\matlabtextC $0$}%
\psfrag{018}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{019}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> fig7a.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{009}[tc][tc]{\matlabtextA $ \gamma_\phi $}%
\psfrag{010}[bc][bc]{\matlabtextA $ \gamma_{\rm b} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $10^{0}$}%
\psfrag{001}[ct][ct]{\matlabtextB $10^{1}$}%
\psfrag{002}[ct][ct]{\matlabtextB $10^{2}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{004}[rc][rc]{\matlabtextB $10^{1}$}%
\psfrag{005}[rc][rc]{\matlabtextB $10^{2}$}%
\psfrag{006}[rc][rc]{\matlabtextB $10^{3}$}%
\psfrag{007}[rc][rc]{\matlabtextB $10^{4}$}%
\psfrag{008}[rc][rc]{\matlabtextB $10^{5}$}%
%
%% </ytick>

==> fig7b.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{010}[tc][tc]{\matlabtextA $ \gamma_\phi $}%
\psfrag{011}[bc][bc]{\matlabtextA $ \gamma_{\rm b} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $10^{2}$}%
\psfrag{001}[ct][ct]{\matlabtextB $10^{3}$}%
\psfrag{002}[ct][ct]{\matlabtextB $10^{4}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextB $10^{2}$}%
\psfrag{004}[rc][rc]{\matlabtextB $10^{3}$}%
\psfrag{005}[rc][rc]{\matlabtextB $10^{4}$}%
\psfrag{006}[rc][rc]{\matlabtextB $10^{5}$}%
\psfrag{007}[rc][rc]{\matlabtextB $10^{6}$}%
\psfrag{008}[rc][rc]{\matlabtextB $10^{7}$}%
\psfrag{009}[rc][rc]{\matlabtextB $10^{8}$}%
%
%% </ytick>

==> fig8a.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{013}[tc][tc]{\matlabtextA $ {\rm sgn}(z)\log_{10}(\gamma_\phi) $}%
\psfrag{014}[bc][bc]{\matlabtextA $ \omega(z)/\omega'_{\rm p0} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 4$}%
\psfrag{001}[ct][ct]{\matlabtextB $\matlabfragNegXTick 3$}%
\psfrag{002}[ct][ct]{\matlabtextB $\matlabfragNegXTick 2$}%
\psfrag{003}[ct][ct]{\matlabtextB $\matlabfragNegXTick 1$}%
\psfrag{004}[ct][ct]{\matlabtextB $0$}%
\psfrag{005}[ct][ct]{\matlabtextB $1$}%
\psfrag{006}[ct][ct]{\matlabtextB $2$}%
\psfrag{007}[ct][ct]{\matlabtextB $3$}%
\psfrag{008}[ct][ct]{\matlabtextB $4$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{010}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{011}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{012}[rc][rc]{\matlabtextB $10^{1}$}%
%
%% </ytick>

==> fig8b.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{014}[tc][tc]{\matlabtextA $ {\rm sgn}(z')\log_{10}(\gamma'_\phi) $}%
\psfrag{015}[bc][bc]{\matlabtextA $ \omega'(z')/\omega'_{\rm p0} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 2$}%
\psfrag{001}[ct][ct]{\matlabtextB $\matlabfragNegXTick 1$}%
\psfrag{002}[ct][ct]{\matlabtextB $0$}%
\psfrag{003}[ct][ct]{\matlabtextB $1$}%
\psfrag{004}[ct][ct]{\matlabtextB $2$}%
\psfrag{005}[ct][ct]{\matlabtextB $3$}%
\psfrag{006}[ct][ct]{\matlabtextB $4$}%
\psfrag{007}[ct][ct]{\matlabtextB $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{009}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{010}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{011}[rc][rc]{\matlabtextB $10^{1}$}%
\psfrag{012}[rc][rc]{\matlabtextB $10^{2}$}%
\psfrag{013}[rc][rc]{\matlabtextB $10^{3}$}%
%
%% </ytick>

==> fig9.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{018}[tc][tc]{\matlabtextA $ {\rm sgn}(z')\log_{10}(\gamma'_\phi) $}%
\psfrag{019}[bc][bc]{\matlabtextA $ \omega'(z')/\omega'_{\rm p0} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.5$}%
\psfrag{001}[ct][ct]{\matlabtextB $0$}%
\psfrag{002}[ct][ct]{\matlabtextB $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextB $1$}%
\psfrag{004}[ct][ct]{\matlabtextB $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextB $2$}%
\psfrag{006}[ct][ct]{\matlabtextB $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextB $3$}%
\psfrag{008}[ct][ct]{\matlabtextB $3.5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextB $10^{-6}$}%
\psfrag{010}[rc][rc]{\matlabtextB $10^{-5}$}%
\psfrag{011}[rc][rc]{\matlabtextB $10^{-4}$}%
\psfrag{012}[rc][rc]{\matlabtextB $10^{-3}$}%
\psfrag{013}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{014}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{015}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{016}[rc][rc]{\matlabtextB $10^{1}$}%
\psfrag{017}[rc][rc]{\matlabtextB $10^{2}$}%
%
%% </ytick>
